Style-Friendly SNR Sampler for Style-Driven Generation

Recent text-to-image diffusion models generate high-quality images but struggle to learn new, personalized styles, which limits the creation of unique style templates. In style-driven generation, users typically supply reference images exemplifying the desired style, together with text prompts that specify desired stylistic attributes. Previous approaches popularly rely on fine-tuning, yet it often blindly utilizes objectives and noise level distributions from pre-training without adaptation. We discover that stylistic features predominantly emerge at higher noise levels, leading current fine-tuning methods to exhibit suboptimal style alignment. We propose the Style-friendly SNR sampler, which aggressively shifts the signal-to-noise ratio (SNR) distribution toward higher noise levels during fine-tuning to focus on noise levels where stylistic features emerge. This enhances models' ability to capture novel styles indicated by reference images and text prompts. We demonstrate improved generation of novel styles that cannot be adequately described solely with a text prompt, enabling the creation of new style templates for personalized content creation.

==> tab/rebuttal_table.tex <==
\begin{table}[t!]
    \setlength{\tabcolsep}{4pt}
    \centering
    \resizebox{0.47\textwidth}{!}{%
        \begin{tabular}{l|l|ccc}
            \hline
            \multirow{2}{*}{Method} & \multirow{2}{*}{Model} & \multicolumn{3}{c}{Metrics} \\
            \cline{3-5}
            & & DINO $\uparrow$ & CLIP-I $\uparrow$ & CLIP-T $\uparrow$ \\
            \hline
            Uniform $t$ & SDXL & 0.542 & 0.721 & 0.331 \\
            \textbf{Style-friendly} & SDXL & \cellcolor{blue!10}0.565 & \cellcolor{blue!10}0.735 & \cellcolor{blue!10}0.333 \\
            \hline
            $\mu=-6, ~\sigma=3$ & SD3.5 & 0.469 & 0.691 & 0.351 \\
            $\mu=-6, ~\sigma=4$ & SD3.5 & 0.461 & 0.685 & 0.351 \\
            DCO & SD3.5 & 0.399 & 0.661 & \cellcolor{blue!10}0.355 \\
            \textbf{Style-friendly}+DCO & SD3.5 & 0.478 & 0.695 & 0.351 \\
            \textbf{Style-friendly} & SD3.5 & \cellcolor{blue!10}0.489 & \cellcolor{blue!10}0.698 & 0.349 \\
            \hline
            SD3 Sampler (4$\times$ LoRA)  & FLUX-dev & 0.426 & 0.668 & \cellcolor{blue!10}0.345 \\
            SD3 Sampler (2$\times$ Optimization)  & FLUX-dev & 0.446 & 0.676 & 0.342 \\
            \textbf{Style-friendly} & FLUX-dev & \cellcolor{blue!10}0.461 & \cellcolor{blue!10}0.686 & 0.344 \\
            \hline
        \end{tabular}%
    }
    \caption{\textbf{Additional quantitative results.} (\textcolor{blue}{R1}, \textcolor{orange}{R2}, \textcolor{violet}{R3})}
    \vspace{-1em}
    \label{tab:rebuttal}
\end{table}

==> tab/snr_compare.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{c | c | c}
\hline
 & Flux and SD3 & SDXL \\
\hline
\rule{0pt}{3.5ex} $p(\lambda_t)$ 
            & \multicolumn{2}{c}{$\lambda_t \sim \mathcal{N}(\mu_{\text{style}}, \sigma_{\text{style}}^2)$} 
            \\
            \hline
\rule{0pt}{3.5ex} $\lambda_t$ & $2\log(\tfrac{1-t}{t})$ 
            & $\log(\tfrac{\alpha_t}{1-\alpha_t})$ 
            \\
            \hline
\rule{0pt}{3.5ex} $t$ 
            & $\frac{1}{\,1 + \exp\!\bigl(\tfrac{\lambda_t}{2}\bigr)}$ 
            & $\underset{\tau \in \{0,\ldots,T-1\}}{\mathrm{argmin}}\;|\alpha_\tau - \alpha_t|$ \\
\hline
\end{tabular}
\caption{\textcolor{red}{Comparison of log-SNR parameterizations and the style-friendly sampler.}}
\label{tab:snr_comparison}
\end{table}

